Estimating Approximate Incentive Compatibility

In practice, most mechanisms for selling, buying, matching, voting, and so on are not incentive compatible. We present techniques for estimating how far a mechanism is from incentive compatible. Given samples from the agents' type distribution, we show how to estimate the extent to which an agent can improve his utility by misreporting his type. We do so by first measuring the maximum utility an agent can gain by misreporting his type on average over the samples, assuming his true and reported types are from a finite subset -- which our technique constructs -- of the type space. The challenge is that by measuring utility gains over a finite subset of the type space, we might miss type pairs $\theta$ and $\hat{\theta}$ where an agent with type $\theta$ can greatly improve his utility by reporting type $\hat{\theta}$. Indeed, our primary technical contribution is proving that the maximum utility gain over this finite subset nearly matches the maximum utility gain overall, despite the volatility of the utility functions we study. We apply our tools to the single-item and combinatorial first-price auctions, generalized second-price auction, discriminatory auction, uniform-price auction, and second-price auction with spiteful bidders.

==> simulations.tex <==
We now present several experiments illustrating the strength of our diserpersion-based estimation technique. We choose mechanisms $M$ and distributions $\dist$ where we can evaluate the expression \begin{equation}\max_{\theta_i, \hat{\theta}_i \in \Theta_i}\left\{\E_{\vec{\theta}_{-i} \sim \dist_{-i}}\left[u_{i, M}\left(\theta_i, \hat{\theta}_i, \vec{\theta}_{-i}\right) - u_{i, M}\left(\theta_i,\theta_i, \vec{\theta}_{-i}\right)\right]\right\}.\label{eq:experiments}\end{equation} This expression can be challenging or even impossible to evaluate even with knowledge of $\dist$.

\begin{figure}
\centering
\begin{subfigure}{0.47\textwidth}
\includegraphics[width=\linewidth]{3FP} \centering
\caption{First-price auction with 3 bidders.}
\label{fig:FP_exp}
\end{subfigure}\qquad
\begin{subfigure}{0.47\textwidth}
\includegraphics[width=\linewidth]{3SP}\centering
\caption{Second-price auction with 3 spiteful bidders.}
\label{fig:SP_exp}
\end{subfigure}
\begin{subfigure}{0.47\textwidth}
\includegraphics[width=\linewidth]{5FP} \centering
\caption{First-price auction with 5 bidders.}
\label{fig:FP_exp}
\end{subfigure}\qquad
\begin{subfigure}{0.47\textwidth}
\includegraphics[width=\linewidth]{5SP}\centering
\caption{Second-price auction with 5 spiteful bidders.}
\label{fig:SP_exp}
\end{subfigure}
\caption{Plots illustrating our estimates converging to the true incentive compatibility approximation factors.} 
\label{fig:exp}
\end{figure}

We analyze the first-price single-item auction with $n \in \{3,5\}$ and the second-price auction with $n \in \{3,5\}$, $\alpha_1 = 1/2$, and $\alpha_2 = \alpha_3 = 0$. In Appendix~\ref{app:exp}, we also show plots for the case where $n = 10$. When there are fewer bidders, each bidder can generally gain more utility by bidding strategically, so Equation~\eqref{eq:experiments} will be larger. In all settings, the values are drawn i.i.d. from Uniform(0,1). Under the the first-price auction with $n = 3$, Equation~\eqref{eq:experiments} equals $0.15$. Under the the first-price auction with $n = 5$, Equation~\eqref{eq:experiments} equals $0.08$. Under the the second-price auction with $n = 3$, Equation~\eqref{eq:experiments} equals $0.05$. Finally, under the the second-price auction with $n = 5$, Equation~\eqref{eq:experiments} equals $0.03$. These values correspond to the horizontal lines in Figure~\ref{fig:exp}.
In all four cases, we range the sample size $N$ up to 360,000 and follow the following procedure. For each bidder $i \in [n]$, we draw $\sample_{-i} = \left\{\vec{\theta}^{\left(1\right)}_{-i}, \dots, \vec{\theta}^{\left(N\right)}_{-i}\right\} \sim \dist_{-i}^N$. In both cases, we know from Lemmas~\ref{lem:FP_discontinuities} and \ref{lem:SP_discontinuities} that the functions
$u_{i, M}\left(\theta_i, \cdot, \vec{\theta}_{-i}^{(1)}\right), \dots, u_{i, M}\left(\theta_i, \cdot, \vec{\theta}_{-i}^{(N)}\right)$ are 1-Lipschitz and their discontinuities fall within the set $T_{-i} = \left\{\norm{\vec{\theta}_{-i}^{(1)}}_{\infty}, \dots, \norm{\vec{\theta}_{-i}^{(N)}}_{\infty}\right\}$. We set $k_i = \lfloor 3\sqrt{N}/2\rfloor$ and we define $w_i$ to be the largest $w$ such that at most $k_i$ points from  $T_{-i}$ fall within any interval of width $2w$. In other words, $w_i = 2\cdot \sup_{w \in (0, 1]} \left\{w : \left|[a, a+w] \cap T_{-i}\right| \leq k_i, \forall a \in [0,1]\right\}$. Figure~\ref{fig:exp} displays the bound from Theorem~\ref{thm:main} (a variation on Theorem~\ref{thm:main_prob}) with $\delta = 0.01$. In all settings, we observe that our estimate quickly converges to the true incentive compatibility approximation factor.
